ZynqParrot: A Scale-Down Approach to Cycle-Accurate, FPGA-Accelerated Co-Emulation

As processors increase in complexity, costs grow even more rapidly, both for functional verification and performance validation. Most often, silicon characterizations comprise simple performance counters, which are aggregated and separated to tell a story. Based on these inferences, performance engineers employ microarchitectural simulation to inspect deeply into the core. Unfortunately, dramatically longer runtimes make simulation infeasible for long workloads. We propose a Scale-Down approach to modelling and validation. Rather than up-sizing a prototyping platform to fit large and complex system designs, we show that it can be more accurate, faster, and more economical to decompose a system into manageable sub-components that can be prototyped independently. By carefully designing the prototyping interface, it is possible to adhere to strict non-interference of the Device Under Test (DUT). This allows architects to have the best of both worlds: the speed of FPGA acceleration while eliminating the inaccuracies of Scale-Out and the inherent costs of Scale-Up. In this work, we present ZynqParrot: a Scale-Down FPGA-based modelling platform, capable of executing non-interfering, cycle-accurate co-emulations of arbitrary RTL designs. ZynqParrot is capable of verifying functionality and performance with arbitrary granularity. We also provide case studies using ZynqParrot to analyze the full-stack performance of an open-source RISC-V processor.

==> 03-software/figs/speedup.tex <==
\begin{table}
    \centering
    \caption{Speedup}
    \resizebox{\columnwidth}{!}{%

\begin{tabular}{|l|l|l|l|}
\hline
Framework                                                                                                      & \begin{tabular}[c]{@{}l@{}}Co-simulation\\ Speed (MIPS)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Absolute\\ Speedup\end{tabular} & \begin{tabular}[c]{@{}l@{}}Relative\\ Speedup\end{tabular} \\ \hline
\begin{tabular}[c]{@{}l@{}}Dromajo standalone simulation\\ (on single-core x86\_64 @3.2 GHz)\end{tabular}      &                                                                     &                                                            &                                                            \\ \hline
Verilator Simulation without Dromajo                                                                           &                                                                     &                                                            &                                                            \\ \hline
Verilator with Dromajo co-simulation                                                                            & 0.000177                                                            & 1.0x                                                       &                                                            \\ \hline
VCS with Dromajo co-simulation                                                                                  & 0.001477                                                            & 8.34x                                                      &                                                            \\ \hline
\begin{tabular}[c]{@{}l@{}}Emulation with Dromajo co-simulation\\ (Baseline)\end{tabular}                       & 0.192                                                               & 1084x                                                      & 1x                                                         \\ \hline
Emulation with SIMD reads into P-Shell                                                                              & 0.273                                                               & 1542x                                                      & 42.18\%                                                    \\ \hline
\begin{tabular}[c]{@{}l@{}}Emulation with asynchronous AXI bus\\ (Core @40 MHz, AXI bus @160 MHz)\end{tabular} & 0.52                                                                & 2937x                                                      & 170\%                                                      \\ \hline
\end{tabular}
    \label{fig:03-speedup}
    }
\end{table}


==> 04-syseval/figs/coremark_speeds.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\begin{tabular}{|l|l|l|r|r|r|}
\hline
\rowcolor[HTML]{C0C0C0} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{C0C0C0}{\color[HTML]{000000} Framework}}                                                                                                                                       & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}{\color[HTML]{000000} \begin{tabular}[c]{@{}c@{}}Co/simulation\\ Speed (MIPS)\end{tabular}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}{\color[HTML]{000000} \begin{tabular}[c]{@{}c@{}}FPGA\\ Speedup\end{tabular}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}{\color[HTML]{000000} \begin{tabular}[c]{@{}c@{}}Cycles\\ Simulated\end{tabular}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}{\color[HTML]{000000} \begin{tabular}[c]{@{}c@{}}Instructions\\ Retired\end{tabular}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}{\color[HTML]{000000} \begin{tabular}[c]{@{}c@{}}Wall Clock\\ Time (s)\end{tabular}}} \\ \hline
\begin{tabular}[c]{@{}l@{}}Dromajo standalone simulation\\ (on single-core x86\_64 @3.2 GHz)\\   + without tracing\\   + with tracing (henceforth)\end{tabular}                                                      & \begin{tabular}[c]{@{}l@{}}16.35\\ 0.59\end{tabular}                                                                                     & \begin{tabular}[c]{@{}l@{}}-\\ -\end{tabular}                                                                              & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}-\\ -\end{tabular}}                                                             & \begin{tabular}[c]{@{}r@{}}1,531,979\\ (same)\end{tabular}                                                                         & \begin{tabular}[c]{@{}r@{}}0.098\\ 2.633\end{tabular}                                                                             \\ \hline
\begin{tabular}[c]{@{}l@{}}Standalone Verilator simulation of BP\\ without ZynqParrot setup\end{tabular}                                                                                                             & 0.001136                                                                                                                                 & 1x                                                                                                                         & 1,885,467                                                                                                                      & 1,532,698                                                                                                                          & 1348.620                                                                                                                          \\ \hline
\begin{tabular}[c]{@{}l@{}}Verilator Simulation of BP \\ with Zynq-Parrot setup (henceforth)\\ (without Dromajo cosimulation)\\ + with Dromajo cosimulation and \\    clock gating enabled (henceforth)\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.001682\\ \\ 0.000112\end{tabular}                                                                           & \begin{tabular}[c]{@{}l@{}}1.48x\\ \\ 0.10x\end{tabular}                                                                   & \begin{tabular}[c]{@{}r@{}}107,556\\ \\ 107,848\end{tabular}                                                                   & \begin{tabular}[c]{@{}r@{}}1,532,166\\ \\ 1,531,967\end{tabular}                                                                   & \begin{tabular}[c]{@{}r@{}}931.843\\ \\ 13,722.234\end{tabular}                                                                   \\ \hline
\begin{tabular}[c]{@{}l@{}}FPGA emulation of BP (Baseline)\\ + with SIMD reads into PL\\ + with asynchronous AXI bus\\    BP @40 MHz, AXI bus @160 MHz\end{tabular}                                                  & \begin{tabular}[c]{@{}l@{}}0.190269\\ 0.268102\\ 0.429813\end{tabular}                                                                   & \begin{tabular}[c]{@{}l@{}}167x\\ 236x\\ 378x\end{tabular}                                                                 & \begin{tabular}[c]{@{}r@{}}108,269\\ 108,674\\ 108,583\end{tabular}                                                            & \begin{tabular}[c]{@{}r@{}}1,531,952\\ (same)\\ (same)\end{tabular}                                                                & \begin{tabular}[c]{@{}r@{}}8.051\\ 5.714\\ 3.564\end{tabular}                                                                     \\ \hline
\end{tabular}
\end{table}


==> 04-syseval/figs/sim_speed.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.45\textwidth]{04-syseval/figs/fake/sim_speed.png}
    \caption{Simulation Speed}
    \label{fig:04-syseval-sim_speed}
    \Description[]{}
\end{figure}


==> 04-syseval/figs/tco.tex <==

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.4\textwidth]{04-syseval/figs/fake/tco.png}
    \caption{SPEC/Dollar/Day}
    \label{fig:04-syseval-tco}
    \Description[]{}
\end{figure}


==> 04-syseval/section.tex <==

\iffalse
\section{System Evaluation}
\bsgsummary{This is evaluating the performance of the system, bottlenecks and possible speedups}
% TODO: Include if ready
%\input{04-syseval/figs/sim_speed}
\input{04-syseval/figs/tco}

% if speed of simulation is an argument, we need to present the ability to checkpoinnt intermediate states and restore in simulation -- Anoop
\fi

==> 05-duteval/figs/blackparrot_opt.tex <==
\begin{figure*}[!t]
\centering
%\subfloat[\blackparrot{} Pre-Opt]{\includegraphics[width=2.5in]{05-duteval/figs/fake/blackparrot_preopt.png}
%\label{fig:05-duteval-blackparrot_preopt}}
%\hfil
%\subfloat[\blackparrot{} Post-Op]{\includegraphics[width=2.5in]{05-duteval/figs/fake/blackparrot_postopt.jpg}
%\label{fig:05-duteval-blackparrot_postopt}}
%\caption{Showing how we used \projectname{} to great success} \label{fig_sim}
\Description[]{}
\end{figure*}

==> 05-duteval/section.tex <==
\iffalse
\section{Case Study: \blackparrot Evaluation}
\bsgsummary{This is describing a performance analysis of \blackparrot{} exposing a potential optimization}
\input{05-duteval/figs/blackparrot_opt}
\fi

==> 06-validation/figs/accuracy.tex <==

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.4\textwidth]{06-validation/figs/fake/accuracy.png}
    \caption{Accuracy of our approach vs others}
    \label{fig:06-validation-accuracy}
    \Description[]{}
\end{figure}


==> 06-validation/section.tex <==
\iffalse
\section{Validation}
\bsgsummary{This is demonstrating the accuracy of \projectname{} and comparing against misattributed stalls in other systems.}
\input{06-validation/figs/accuracy}
\fi

==> 97-future/section.tex <==
\section{Future Work}
While \projectname{} has been successfully used for classwork, academic research and industrial prototyping, in this section we consider several directions to enhance versatility and robustness:
\begin{enumerate}
    \item While Scale-Down methodology greatly benefits prototyping iteration time, subdividing the design into co-emulatable subcomponents is generally a manual process. Automatically partitioning commercial-size architecturables could lead to faster full-design iterations, detecting bugs earlier in the design schedule.
    \item Although \projectname{} currently supports DRAM, UART and Ethernet as well as a small set of demonstration AXI-lite masters and clients, we anticipate community development of a diverse open-source library of functional and timing models for common peripherals.
    \item \projectname{} was intentionally developed to minimize dependence on proprietary vendor IP. While current implementations use Xilinx Zynq and Virtex parts, only a small subset of the infrastructure (< 100 lines of TCL) must be ported to support new boards. We hope in the future to support Intel and Lattice alternatives to broaden the reach of \projectname{} to teams which are bound to these vendors. 
\end{enumerate}


==> 99-acknowledgements/section.tex <==

\section*{Acknowledgment}
\bsgsummary{We acknowledge funding sponsors and various contributing non-authors to \projectname{}}

